Efficient Decision Procedures for RNmatrix Semantics

Logical matrices provide a semantic framework in which connectives are interpreted by deterministic truth-functions. While elegant, this approach is often too restrictive to capture the semantics of many non-classical logics. Non-deterministic matrices (Nmatrices) generalise ordinary matrices by allowing connectives to return a set of possible truth values rather than a unique one, thereby increasing expressive power. Restricted non-deterministic matrices (RNmatrices) further refine this framework by imposing constraints on the rows of Nmatrices, filtering out "unsound" rows and retaining only "valid" ones. This yields a more expressive semantic framework that has been successfully used to provide sound and complete semantics for a wide range of logics, including paraconsistent, intuitionistic, and modal logics. Despite these advances, no efficient decision procedures based on RNmatrix semantics have been proposed. In this paper, we develop automated theorem provers based on RNmatrices by encoding their semantics as Satisfiability Modulo Theories (SMT) problems. The resulting provers decide validity and construct countermodels, achieving state-of-the-art performance for paraconsistent logics and competitive results for intuitionistic and modal logics.

==> eptcsdata.tex <==
\providecommand{\firstpage}{167}
\providecommand{\publicationstatus}{V. de Paiva; T.A. de Lima (Eds.): 21st International Symposium\\ on Logical and Semantic Frameworks, with Applications (LSFA 2026)\\
EPTCS 449, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.449.11}{10.4204/EPTCS.449.11}}
\pdfoutput=1

